Stochastic Gradient Descent in Hilbert Scales: Smoothness, Preconditioning and Earlier Stopping

Stochastic Gradient Descent (SGD) has become the method of choice for solving a broad range of machine learning problems. However, some of its learning properties are still not fully understood. We consider least squares learning in reproducing kernel Hilbert spaces (RKHSs) and extend the classical SGD analysis to a learning setting in Hilbert scales, including Sobolev spaces and Diffusion spaces on compact Riemannian manifolds. We show that even for well-specified models, violation of a traditional benchmark smoothness assumption has a tremendous effect on the learning rate. In addition, we show that for miss-specified models, preconditioning in an appropriate Hilbert scale helps to reduce the number of iterations, i.e. allowing for "earlier stopping".

==> app-numerics.tex <==
%Here we give some more details for the empirical studies we conducted. 

%{\bf Stepsize depends linearly on the batchsize: } 
%The minimizer $f_\cH$ is chosen to be a sum of Gaussians as in Eq. \ref{eq:gauss}. 
%We perform one pass SGD, i.e. $T = n/b$, with $n=3\cdot 10^3$ in the Sobolev space $H^{3+\frac{1}{2}}(\mbr)$ by utilizing the \emph{Mat\'ern} Kernel of order $3$, 
%see below for a precise description. Then our model is well-specified. 
%The result is given in  Fig. \ref{fig:3}. As predicted by Cor. \ref{cor:ratesSGD}, \ref{cor:ratesSGD2}, performance remains largely constant as 
%$\gamma \cdot b$ remains constant. 


%\begin{figure}[h]
%  \centering
%  \includegraphics[width=0.34\columnwidth, height=0.17\textheight]{fig02_norm(2)}%{fig_testError_GaussKernel} %Simu 10 {fig02}
% \caption{{\small Stepsize depends linearly on the batchsize.}}
%\label{fig:3}
%\end{figure}

A particular family of kernels on $\mbr^d$ leading to the family of Sobolev spaces  $(H^s(\mbr^d))_{s\geq 0}$ are the 
translation invariant \emph{Mat\'ern Kernels} \cite{yang2017frequentist}. Let 
\[ k_\alpha(t):= \frac{\sigma^2}{2^{\alpha-1}\Gamma(\alpha)}\cdot \left(\frac{2\sqrt{\alpha}}{\theta} t\right)^\alpha H_\alpha \left(\frac{2\sqrt{\alpha}}{\theta} t\right)\;, \]
where $\theta>0$, $\sigma >0$, $\alpha >0$ and with $H_\alpha$ the \emph{modified Bessel function of the second kind}. Then we set 
\[ K_\alpha( x, x'):=k_\alpha(||x-x'||_2) \;, \quad  x, x' \in \mbr^d \;. \]
Denoting the RKHS associated to $K_\alpha$ as $\cH_\alpha$, it is well known that  
\[ \cH_\alpha \cong H^{\alpha+d/2}(\mbr^d) \;.\] 
Moreover, the eigenvalues $(\mu_j)_{j=1}^\infty$ of the associated kernel integral operator satisfy 
$\mu_j \asymp j^{-2(\alpha+d/2)}$, for $\alpha>1-d/2$.



==> macros_nicole.tex <==
%Packages standard

%\RequirePackage{wasysym }
%\RequirePackage[isolatin]{inputenc}
\RequirePackage{comment}
\RequirePackage{graphicx}
%\usepackage{amsmath}%,amsfonts}
\RequirePackage{color}
%Theoremes

\usepackage{colortbl}
\usepackage{xcolor}

\usepackage{mathrsfs,amsfonts,amssymb,amstext,bm,bbm,dsfont,pifont,amscd,
            amsthm,stmaryrd,euscript}
            
\usepackage{mathtools}


\definecolor{blue}{rgb}{0.6, 0.4, 1.0} %{0.0,0.0,0.55}
%\definecolor{blue}{rgb}{0.0,0.0,0.55}
\definecolor{red}{rgb}{0.75,0.0,0.0}
\definecolor{green}{rgb}{0.0,0.5,0.0}
\definecolor{bluebell}{rgb}{0.64, 0.64, 0.82}
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{awesome}{rgb}{1.0, 0.13, 0.32}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
\definecolor{nic}{rgb}{0.6, 0.4, 1.0} %{0.0,0.0,0.55}

\newcommand{\magenta}{\color{magenta}}
\newcommand{\blue}{\color{blue}}
\newcommand{\green}{\color{green}}
\newcommand{\red}{\color{red}}
 

%\ifx \skiptheorems \thiscommandisnotdefinedtralala  
                 %teste si \skiptheorems est non-defini

\RequirePackage{amsthm}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}
% 
%\theoremstyle{remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{example}[theorem]{Example}
%\newtheorem{example}{Example}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\no}{\nonumber}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}


%\DeclareMathOperator{\supp}{supp}

\def\argmax{\operatornamewithlimits{arg\,max}}
\def\argmin{\operatornamewithlimits{arg\,min}}


% Fonts

\newcommand{\mtc}{\mathcal}
\newcommand{\mbf}{\mathbf}

% Some black magic to remove annoying extra spaces before/after \left* and \right*

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}


% Accents tildes over/underline etc

\newcommand{\wt}[1]{{\widetilde{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}

% Delimiteurs divers

\RequirePackage{xstring}

\newcommand{\ind}[1]{{\mbf{1}\{#1\}}}
\newcommand{\paren}[2][a]{%
\IfEqCase{#1}{%
{a}{\left(#2\right)}%
{0}{(#2)}%
{1}{\big(#2\big)}%
{2}{\Big(#2\Big)}%
{3}{\bigg(#2\bigg)}%
{4}{\Bigg(#2\Bigg)}%
}[\PackageError{paren}{Undefined option to paren: #1}{}]%
}
\newcommand{\norm}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\lVert#2\right\rVert}%
{0}{\lVert#2\rVert}%
{1}{\big\lVert#2\big\rVert}%
{2}{\Big\lVert#2\Big\rVert}%
{3}{\bigg\lVert#2\bigg\rVert}%
{4}{\Bigg\lVert#2\Bigg\rVert}%
}[\PackageError{norm}{Undefined option to norm: #1}{}]%
}
\newcommand{\brac}[2][a]{%
\IfEqCase{#1}{%
{a}{\left[#2\right]}%
{0}{[#2]}%
{1}{\big[#2\big]}%
{2}{\Big[#2\Big]}%
{3}{\bigg[#2\bigg]}%
{4}{\Bigg[#2\Bigg]}%
}[\PackageError{brac}{Undefined option to brac: #1}{}]%
}
\newcommand{\inner}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\langle#2\right\rangle}%
{0}{\langle#2\rangle}%
{1}{\big\langle#2\big\rangle}%
{2}{\Big\langle#2\Big\rangle}%
{3}{\bigg\langle#2\bigg\rangle}%
{4}{\Bigg\langle#2\Bigg\rangle}%
}[\PackageError{inner}{Undefined option to inner: #1}{}]%
}
\newcommand{\abs}[2][a]{
\IfEqCase{#1}{%
{a}{\left\vert#2\right\rvert}%
{0}{\vert#2\rvert}%
{1}{\big\vert#2\big\rvert}%
{2}{\Big\vert#2\Big\rvert}%
{3}{\bigg\vert#2\bigg\rvert}%
{4}{\Bigg\vert#2\Bigg\rvert}%
}[\PackageError{inner}{Undefined option to abs: #1}{}]%
}



%\newcommand{\set}[1]{\left\{#1\right\}}


\newcommand{\eins}{\boldsymbol{1}}


%\newcommand{\var}[2][a]{{\rm Var}\brac[#1]{#2}}
\newcommand{\cov}[2][a]{{\rm Cov}\brac[#1]{#2}} 
%\newcommand{\e}[2][a]{\mbe\brac[#1]{#2}}
\newcommand{\ee}[3][a]{\mbe_{#2}\brac[#1]{#3}}
\newcommand{\prob}[2][a]{\mbp\brac[#1]{#2}}
\newcommand{\probb}[3][a]{\mbp_{#2}\brac[#1]{#3}}


% Operateurs

\def\argmin{\mathop{\rm Arg\,Min}\limits}
\def\argmax{\mathop{\rm Arg\,Max}\limits}
\def\sgn{\mathop{\rm Sgn}\limits}
\def\tr{\mathop{\rm Tr}\limits}


% abbrev lettres grecques

\newcommand{\al}{\alpha}
\newcommand{\lam}{\lambda}
%\newcommand{\om}{\omega}
\newcommand{\eps}{\varepsilon}

% abbrev lettres mathcal

\def\cA{{\mtc{A}}}
\def\cB{{\mtc{B}}}
\def\cC{{\mtc{C}}}
\def\cD{{\mtc{D}}}
\def\cE{{\mtc{E}}}
\def\cF{{\mtc{F}}}
\def\cG{{\mtc{G}}}
\def\cH{{\mtc{H}}}
\def\cI{{\mtc{I}}}
\def\cK{{\mtc{K}}}
\def\cL{{\mtc{L}}}
\def\cM{{\mtc{M}}}
\def\cN{{\mtc{N}}}
\def\cO{{\mtc{O}}}
\def\cP{{\mtc{P}}}
\def\cQ{{\mtc{Q}}}
\def\cR{{\mtc{R}}}
\def\cS{{\mtc{S}}}
\def\cT{{\mtc{T}}}
\def\cU{{\mtc{U}}}
\def\cV{{\mtc{V}}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

% abbrev lettres mathbb

\newcommand{\mbe}{\mathbb{E}}
\newcommand{\mbr}{\mathbb{R}}
\newcommand{\mbp}{\mathbb{P}}
\newcommand{\mbq}{\mathbb{Q}}
\newcommand{\mbi}{\mathbb{I}}
\newcommand{\mbn}{\mathbb{N}}
\newcommand{\mbz}{\mathbb{Z}}
\newcommand{\mbs}{\mathbb{S}}
\newcommand{\mbk}{\mathbb{K}}
\newcommand{\mbg}{\mathbb{G}}
\newcommand{\mbv}{\mathbb{V}}


% abbrev lettres en gras

\newcommand{\bA}{{\mbf{A}}}
\newcommand{\bB}{{\mbf{B}}}
\newcommand{\bD}{{\mbf{D}}}
\newcommand{\bG}{{\mbf{G}}}
\newcommand{\bI}{{\mbf{I}}}
\newcommand{\bJ}{{\mbf{J}}}
\newcommand{\bW}{{\mbf{W}}}
\newcommand{\bX}{{\mbf{X}}}
\newcommand{\bY}{{\mbf{Y}}}
\newcommand{\bZ}{{\mbf{Z}}}


\newcommand{\bp}{{\mbf{p}}}
\newcommand{\boldf}{{\mbf{f}}}
\newcommand{\bx}{{\mbf{x}}}
\newcommand{\by}{{\mbf{y}}}
\newcommand{\bz}{{\mbf{z}}}
\newcommand{\bw}{{\mbf{w}}}
\newcommand{\bv}{{\mbf{v}}}
\newcommand{\bs}{{\mbf{s}}}
\newcommand{\barx}{{\bar{x}}}

% frak

\newcommand{\fP}{{\mathfrak{P}}}
\newcommand{\fK}{{\mathfrak{K}}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

%\newcommand{\red}[1]{\textcolor{red}{#1}}


\newcommand{\nux}{\nu}


% TODO command

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% A command to put notes in a draft


\newcommand{\notice}[1]{\color{magenta} #1}

\newcounter{nbdrafts}
\setcounter{nbdrafts}{0}
\makeatletter
\newcommand{\checknbdrafts}{
\ifnum \thenbdrafts > 0
\@latex@warning@no@line{**********************************************************************}
\@latex@warning@no@line{* The document contains \thenbdrafts \space draft note(s)}
\@latex@warning@no@line{**********************************************************************}
\fi}
\newcommand{\todo}[1]{\addtocounter{nbdrafts}{1}{\color{awesome} #1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{nbnotes}
\setcounter{nbnotes}{0}
\makeatletter
\newcommand{\checknbnotes}{
\ifnum \thenbnotes > 0
\@latex@warning@no@line{**********************************************************************}
\@latex@warning@no@line{* The document contains \thenbnotes \space color note(s)}
\@latex@warning@no@line{**********************************************************************}
\fi}
\newcommand{\note}[1]{\addtocounter{nbnotes}{1}{\color{blue} #1}}%amethyst
\makeatother

